Zero-shot Musical Stem Retrieval with Joint-Embedding Predictive Architectures

In this paper, we tackle the task of musical stem retrieval. Given a musical mix, it consists in retrieving a stem that would fit with it, i.e., that would sound pleasant if played together. To do so, we introduce a new method based on Joint-Embedding Predictive Architectures, where an encoder and a predictor are jointly trained to produce latent representations of a context and predict latent representations of a target. In particular, we design our predictor to be conditioned on arbitrary instruments, enabling our model to perform zero-shot stem retrieval. In addition, we discover that pretraining the encoder using contrastive learning drastically improves the model's performance. We validate the retrieval performances of our model using the MUSDB18 and MoisesDB datasets. We show that it significantly outperforms previous baselines on both datasets, showcasing its ability to support more or less precise (and possibly unseen) conditioning. We also evaluate the learned embeddings on a beat tracking task, demonstrating that they retain temporal structure and local information.

==> tables/downstream.tex <==
\begin{table*}
    \centering
    \caption{
        Influence of our different design choices on various downstream tasks, and comparison with existing baselines.
    }
    \label{tab:downstream}
    {\footnotesize
        \begin{tabular}{lccccccc}
            \toprule
             & GS & GTZAN & \multicolumn{2}{c}{GTZANtempo} & \multicolumn{2}{c}{MTT} & NSynth \\
            Model & Acc\textsuperscript{refined} & Acc & Acc1 & Acc2 & ROC & AP & Acc \\
            \midrule
            CLAP conditioning (6a7099c4) &
            50.0 & 76.7 & 65.3 & 74.3 & 90.5 & 44.0 & 75.5 \\
            +FiLM conditioning (64969267) &
            45.0 & \textbf{78.4} & 45.5 & 49.8 & 90.7 & \textbf{44.4} & 75.6 \\
            +contrastive pretraining (6484864f) &
            58.7 & 55.6 & 68.9 & \textbf{82.6} & 88.0 & 37.7 & 74.5 \\
            +FiLM conditioning (dfe9828d) &
            60.0 & 63.0 & \textbf{70.1} & 82.3 & 88.8 & 39.8 & 76.7 \\
            \textit{no flat} \\
            +contrastive pretraining (990d42bb) &
            59.5 & 61.5 & 66.6 & 81.2 & 88.7 & 39.5 & 74.9 \\
            +FiLM conditioning (0857dce1) &
            61.0 & 72.9 & 69.3 & 79.7 & 89.9 & 42.6 & 75.7 \\
            % +MCL (be32f074) &
            % 60.8 & 58.6 & 88.6 & 39.2 & 74.9 \\
            \midrule
            Contrastive (3ff57432) &
            \textbf{66.4} & 68.9 & 65.9 & 79.1 & 89.4 & 41.6 & \textbf{76.8} \\
            Contrastive no flat (ed948e48) &
            63.5 & 65.3 & 67.9 & 80.7 & 88.5 & 38.6 & 75.1 \\            
            Stem-JEPA \cite{StemJEPA}  (10c99d92)    &
            40.2 & 68.6 & 68.1 & 76.2 & 89.9 & 42.8 & 73.5 \\
            Stem-JEPA CLAP (72fe140f) &
            37.6 & 68.5 & 70.6 & 80.2 & 89.7 & 42.5 & 74.7 \\
            Stem-JEPA w/o cond. (9cb7eb0d) &
            36.8 & 72.5 & 61.4 & 69.4 & 90.1 & 42.9 & 75.0 \\
            Transformer (a12e52d8) &
            46.0 & 68.1 & 18.6 & 21.0 & 89.9 & 42.7 & 73.3 \\
            \midrule
            MULE \cite{MULE} &
            64.9 & 75.5 & & & 91.2 & 40.1 & 74.6 \\
            %MULE &
            %50.8 & 68.6 & 90.5 & 38.9 & 71.4 \\
            Jukebox \cite{Jukebox} &
            63.8 & 77.9 & & & \textbf{91.4} & 40.6 & 70.4 \\
            \bottomrule
        \end{tabular}
    }
\end{table*}

==> tables/downstream2.tex <==
\begin{table}
    \centering
    \caption{
        Influence of our different design choices on various downstream tasks, and comparison with existing baselines.
    }
    \label{tab:downstream}
    {%\footnotesize
        \begin{tabular}{lccccccc}
            \toprule
             & GS & GTZAN & \multicolumn{2}{c}{GTZANtempo} & \multicolumn{2}{c}{MTT} & NSynth \\
            Model & Acc\textsuperscript{refined} & Acc & Acc1 & Acc2 & ROC & AP & Acc \\
            \midrule
            Contrastive baseline &
            \textbf{66.4} & 68.9 & 65.9 & 79.1 & 89.4 & 41.6 & \textbf{76.8} \\
            %Contrastive no flat (ed948e48) &
            %63.5 & 65.3 & 67.9 & 80.7 & 88.5 & 38.6 & 75.1 \\            
            Stem-JEPA \cite{StemJEPA} &
            40.2 & 68.6 & 68.1 & 76.2 & 89.9 & 42.8 & 73.5 \\
            \midrule
            +CLAP conditioning &
            50.0 & 76.7 & 65.3 & 74.3 & 90.5 & 44.0 & 75.5 \\
            %+FiLM conditioning (64969267) &
            %45.0 & \textbf{78.4} & 45.5 & 49.8 & 90.7 & \textbf{44.4} & 75.6 \\
            +contrastive pretraining &
            58.7 & 55.6 & 68.9 & \textbf{82.6} & 88.0 & 37.7 & 74.5 \\
            +FiLM conditioning &
            60.0 & 63.0 & \textbf{70.1} & 82.3 & 88.8 & 39.8 & 76.7 \\
            % \textit{no flat} \\
            % +contrastive pretraining (990d42bb) &
            % 59.5 & 61.5 & 66.6 & 81.2 & 88.7 & 39.5 & 74.9 \\
            % +FiLM conditioning (0857dce1) &
            % 61.0 & 72.9 & 69.3 & 79.7 & 89.9 & 42.6 & 75.7 \\
            % +MCL (be32f074) &
            % 60.8 & 58.6 & 88.6 & 39.2 & 74.9 \\
            % \midrule
            % Stem-JEPA CLAP (72fe140f) &
            % 37.6 & 68.5 & 70.6 & 80.2 & 89.7 & 42.5 & 74.7 \\
            % Stem-JEPA w/o cond. (9cb7eb0d) &
            % 36.8 & 72.5 & 61.4 & 69.4 & 90.1 & 42.9 & 75.0 \\
            % Transformer (a12e52d8) &
            % 46.0 & 68.1 & 18.6 & 21.0 & 89.9 & 42.7 & 73.3 \\
            \midrule
            MULE \cite{MULE} &
            64.9 & 75.5 & & & 91.2 & 40.1 & 74.6 \\
            %MULE &
            %50.8 & 68.6 & 90.5 & 38.9 & 71.4 \\
            Jukebox \cite{Jukebox} &
            63.8 & 77.9 & & & \textbf{91.4} & 40.6 & 70.4 \\
            \bottomrule
        \end{tabular}
    }
\end{table}

==> tables/moises.tex <==
\begin{table*}
    \centering
    \caption{Retrieval performances of our model on the MoisesDB dataset. All metrics are in percentages.}
    \label{tab:retrieval}
    {\footnotesize
        \begin{tabular}{lccccccc}
            \toprule
            & \multicolumn{3}{c}{Recall $\uparrow$} &  & \multicolumn{2}{c}{Normalized Rank $\downarrow$} \\
            %\cline{3-3} \cline{5-5} \cline{7-8} \cline{10-11} \cline{13-13} \cline{15-15}
            Model &
            R@1 & R@5 & R@10 &  & mean & median \\
            \midrule
            \textit{fine conditioning} \\
            CLAP conditioning &
            19.3 & 35.8 & 44.0 &  & 7.2 & 0.7 \\
            +contrastive pretraining (6484864f) &
            12.5 & 45.6 & \textbf{59.3} &  & \textbf{1.9} & 0.3 \\
            +FiLM conditioning (dfe9828d) &
            \textbf{22.0} & \textbf{49.5} & 57.8 &  & 4.5 & \textbf{0.2} \\
            % +MCL (classifier) (be32f074) &
            % 19.0 & 46.9 & 55.6 &  & 7.5 & 0.3 \\
            % +MCL (oracle) &
            %  \\
            \midrule
            \textit{coarse conditioning} \\
            CLAP conditioning &
            18.9 & 37.8 & 46.9 &  & 7.3 & 0.5 \\
            +contrastive pretraining (6484864f) &
            11.1 & 44.5 & 58.1 &  & \textbf{2.1} & 0.3 \\
            +FiLM conditioning (dfe9828d) &
            \textbf{19.2} & \textbf{49.5} & \textbf{60.0} &  & 3.8 & \textbf{0.2} \\
            %+MCL (classifier) (be32f074) &
            %16.1 & 46.3 & 56.4 &  & 5.81 & 0.27 \\
            %+MCL (oracle) &
            %26.4 & 58.5 & 68.6 &  & 3.11 & 0.15 \\
            \midrule
            Contrastive &
             2.7 & 31.2 & 43.3 &  & 7.7 & 0.6 \\
            Stem-JEPA &
             9.9 & 24.1 & 31.6 &  & 11.7 & 1.7 \\
            \bottomrule
        \end{tabular}
    }
\end{table*}

==> tables/musdb.tex <==
\begin{table}
    \centering
    \caption{Retrieval performances of our model on the MUSDB18 dataset. All metrics are in percentages.}
    \label{tab:retrieval}
    {\footnotesize
        \begin{tabular}{lccccccc}
            \toprule
            & \multicolumn{3}{c}{Recall $\uparrow$} &  & \multicolumn{2}{c}{Normalized Rank $\downarrow$} \\
            %\cline{3-3} \cline{5-5} \cline{7-8} \cline{10-11} \cline{13-13} \cline{15-15}
            Model &
            R@1 & R@5 & R@10 &  & mean & median \\
            \midrule
            CLAP conditioning (6a7099c4) &
            33.5 & 63.0 & 74.5 &  &  2.5 &  0.5 \\
            +contrastive pretraining (6484864f) &
            32.2 & \textbf{91.0} & \textbf{96.2} &  &  \textbf{0.6} &  \textbf{0.3} \\
            +FiLM conditioning (dfe9828d) &
            \textbf{38.8} & 89.7 & 95.0 &  &  0.7 &  \textbf{0.3} \\
            %+MCL (classifier) (be32f074) &
            %34.3 & 85.7 & 92.2 &  &  0.9 &  \textbf{0.3} \\
            %+MCL (oracle) &
            %\textbf{51.2} & \textbf{94.3} & \textbf{96.7} &  &  \textbf{0.5} &  \textbf{0.2} \\
            \midrule
            Contrastive (3ff57432) &
             2.2 & 72.5 & 86.0 &  &  1.5 &  0.7 \\
            Stem-JEPA     &
            33.0 & 63.2 & 76.2 &  &  2.0 &  0.5 \\
            \bottomrule
        \end{tabular}
    }
\end{table}
